An Aligned Orbit for the Young Planet V1298 Tau b

The alignment of planetary orbits with respect to the stellar rotation preserves information on their dynamical histories. Measuring this angle for young planets help illuminate the mechanisms that create misaligned orbits for older planets, as different processes could operate over timescales ranging from a few Myr to a Gyr. We present spectroscopic transit observations of the young exoplanet V1298 Tau b; we update the age of V1298 Tau to be $28\pm4$ Myr based on Gaia EDR3 measurements. We observed a partial transit with Keck/HIRES and LBT/PEPSI, and detected the radial velocity anomaly due to the Rossiter-McLaughlin effect. V1298 Tau~b has a prograde, well-aligned orbit, with $\lambda = 4_{-10}^{+7 \circ}$. By combining the spectroscopically-measured $v\sin i_{\star}$ and the phtometrically-measured rotation period of the host star we also find that the orbit is aligned in 3D, $\psi = 8_{-7}^{+4 \circ}$ deg. Finally, we combine our obliquity constraints with a previous measurement for the interior planet V1298 Tau c to constrain the mutual inclination between the two planets to be $i_{\mathrm{mut}}=0^{\circ} \pm 19^{\circ}$. This measurements adds to the growing number of well-aligned planets at young ages, hinting that misalignments may be generated over timescales of longer than tens of Myr. The number of measurements, however, is still small, and this population may not be representative of the older planets that have been observed to date. We also present the derivation of the relationship between $i_{\mathrm{mut}}$, $\lambda$, and $i$ for two planets.

==> gp_protprio_hires.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
{} &       mean &         sd &     hdi\_3\% &     hdi\_97\% &  mcse\_mean &   mcse\_sd &     ess\_bulk &     ess\_tail &     r\_hat \\
\midrule
period        &  24.141341 &   0.000023 &  24.141298 &   24.141385 &   0.000000 &  0.000000 &  5965.607075 &  3931.300517 &  1.000051 \\
t0            &  -0.005427 &   0.001296 &  -0.008042 &   -0.003120 &   0.000017 &  0.000012 &  5487.265493 &  3795.310890 &  0.999812 \\
mean\_spitz    &   0.050990 &   0.045369 &  -0.040393 &    0.130696 &   0.000566 &  0.000501 &  6457.682268 &  3519.741095 &  1.000466 \\
mean\_hires    &  18.987301 &  49.738921 & -73.903162 &  112.310676 &   0.650513 &  0.742112 &  5842.890827 &  3321.063932 &  1.000624 \\
log\_sigma\_rot &   5.525917 &   0.533075 &   4.570491 &    6.539672 &   0.008659 &  0.006415 &  4650.748462 &  2445.639469 &  1.000950 \\
log\_Q0        &   7.653119 &   6.473330 &  -1.751409 &   19.965029 &   0.138749 &  0.100350 &  2372.537290 &  3159.257020 &  1.000151 \\
log\_dQ        &   1.992887 &   9.893170 & -18.069609 &   19.414746 &   0.123409 &  0.152133 &  6434.336147 &  3167.743350 &  0.999827 \\
m\_star        &   1.135137 &   0.047457 &   1.050452 &    1.228125 &   0.000624 &  0.000441 &  5802.712688 &  3621.905375 &  1.000086 \\
r\_star        &   1.406925 &   0.017623 &   1.375033 &    1.441030 &   0.000286 &  0.000203 &  3930.944115 &  3158.665596 &  1.000682 \\
ror           &   0.071998 &   0.000618 &   0.070847 &    0.073131 &   0.000009 &  0.000006 &  4626.205392 &  3170.773750 &  1.000091 \\
r\_pl          &   0.101299 &   0.001741 &   0.098007 &    0.104594 &   0.000028 &  0.000020 &  3871.777007 &  3373.950305 &  0.999765 \\
b             &   0.563932 &   0.025827 &   0.515350 &    0.613040 &   0.000445 &  0.000315 &  3473.687472 &  2602.716947 &  1.000040 \\
u\_star[0]     &   0.543535 &   0.229406 &   0.093268 &    0.925340 &   0.003217 &  0.002286 &  5032.663922 &  3100.213422 &  1.000349 \\
u\_star[1]     &  -0.027872 &   0.272780 &  -0.473508 &    0.473050 &   0.003869 &  0.003909 &  4697.828495 &  2972.263922 &  1.001772 \\
u\_star\_ir[0]  &   0.557989 &   0.144027 &   0.269669 &    0.793776 &   0.002260 &  0.001625 &  3883.100840 &  3647.478831 &  1.000150 \\
u\_star\_ir[1]  &  -0.146108 &   0.178718 &  -0.398195 &    0.202637 &   0.002954 &  0.002432 &  3227.916936 &  2778.152274 &  1.000311 \\
logjit\_spitz  &  -5.941533 &   2.281926 &  -9.759120 &   -2.198497 &   0.037423 &  0.029355 &  3498.414379 &  2428.251489 &  1.000602 \\
jit\_spitz     &   0.018285 &   0.034184 &   0.000045 &    0.090028 &   0.000441 &  0.000345 &  3498.414379 &  2428.251489 &  1.000602 \\
err\_spitz     &   0.601238 &   0.004007 &   0.600000 &    0.606717 &   0.000057 &  0.000040 &  3498.414379 &  2428.251489 &  1.000648 \\
vsini         &  24.773362 &   0.192412 &  24.404368 &   25.121604 &   0.002606 &  0.001843 &  5439.169218 &  3410.288523 &  1.001003 \\
cosi\_st       &   0.084929 &   0.061840 &   0.000015 &    0.196491 &   0.001265 &  0.000894 &  2000.464609 &  1821.394765 &  1.001457 \\
sini\_st       &   0.994440 &   0.007218 &   0.980506 &    1.000000 &   0.000142 &  0.000100 &  2000.464609 &  1821.394765 &  1.001457 \\
i\_st          &  85.116718 &   3.570730 &  78.668164 &   89.999141 &   0.073006 &  0.051796 &  2000.464609 &  1821.394765 &  1.001457 \\
veq           &  24.913143 &   0.261552 &  24.441452 &   25.410837 &   0.004516 &  0.003196 &  3441.039486 &  3562.858289 &  1.000565 \\
a\_r           &  26.061543 &   0.464910 &  25.136114 &   26.873247 &   0.007512 &  0.005313 &  3829.863355 &  3559.044485 &  0.999877 \\
cosi\_pl       &   0.021661 &   0.001346 &   0.019010 &    0.024090 &   0.000023 &  0.000016 &  3426.666974 &  2599.317881 &  0.999887 \\
i\_pl\_deg      &  88.758813 &   0.077128 &  88.619594 &   88.910723 &   0.001321 &  0.000934 &  3426.666974 &  2599.317881 &  0.999887 \\
obliquity\_rad &   0.138430 &   0.268435 &  -0.234580 &    0.739010 &   0.007076 &  0.005225 &  2455.460203 &  1525.551922 &  1.000211 \\
obliquity     &   7.931429 &  15.380195 & -13.440442 &   42.342126 &   0.405444 &  0.299354 &  2455.460203 &  1525.551922 &  1.000211 \\
f             &   0.570509 &   0.248699 &   0.173215 &    0.999639 &   0.002952 &  0.002171 &  6689.040136 &  3077.887995 &  0.999959 \\
\bottomrule
\end{tabular}


==> rvs.tex <==
\begin{tabular}{rrrl}
\toprule
       BJD (d) & RV (m/s) & RV error (m/s) & Instrument \\
\midrule
2458765.926557 &   -268.1 &           11.2 &      HIRES \\
2458774.915387 &    155.3 &            9.6 &      HIRES \\
2458777.016334 &    -36.9 &            9.6 &      HIRES \\

2458781.042264 &     51.9 &            5.7 &      HIRES \\
2458781.036858 &     84.9 &            5.7 &      HIRES \\
2458781.031256 &    101.9 &            6.1 &      HIRES \\
2458781.025654 &    101.6 &            6.0 &      HIRES \\
2458781.015873 &     85.5 &            7.4 &      HIRES \\
2458781.011371 &    116.8 &            6.2 &      HIRES \\
2458781.005688 &    131.2 &            6.2 &      HIRES \\
2458781.000259 &    120.2 &            6.1 &      HIRES \\
2458780.994703 &    144.4 &            5.9 &      HIRES \\
2458780.989101 &    138.3 &            5.8 &      HIRES \\
2458781.047484 &     65.1 &            5.9 &      HIRES \\
2458780.983614 &    151.4 &            5.7 &      HIRES \\
2458780.973360 &    160.5 &            5.8 &      HIRES \\
2458780.968163 &    142.4 &            6.0 &      HIRES \\
2458780.962849 &    138.6 &            5.2 &      HIRES \\
2458780.957653 &    105.6 &            5.5 &      HIRES \\
2458780.952537 &     99.1 &            6.0 &      HIRES \\
2458780.942362 &    103.9 &            5.9 &      HIRES \\
2458780.937189 &    108.9 &            6.0 &      HIRES \\
2458780.931980 &    107.1 &            6.0 &      HIRES \\
2458780.926679 &    132.9 &            5.9 &      HIRES \\
2458780.978394 &    161.8 &            5.8 &      HIRES \\
2458780.921389 &    114.4 &            5.6 &      HIRES \\
2458781.052600 &     54.3 &            5.7 &      HIRES \\
2458781.063041 &     29.5 &            6.0 &      HIRES \\
2458781.156679 &    -85.7 &            6.0 &      HIRES \\
2458781.151806 &    -92.2 &            6.0 &      HIRES \\
2458781.146806 &    -89.2 &            5.9 &      HIRES \\
2458781.141876 &    -75.3 &            6.2 &      HIRES \\
2458781.136909 &    -81.5 &            6.2 &      HIRES \\
2458781.131956 &    -63.8 &            6.2 &      HIRES \\
2458781.057773 &     21.1 &            6.2 &      HIRES \\
2458781.126990 &    -76.0 &            5.7 &      HIRES \\
2458781.116851 &    -53.8 &            6.4 &      HIRES \\
2458781.111492 &    -44.5 &            6.3 &      HIRES \\
2458781.106318 &    -25.4 &            6.0 &      HIRES \\
2458781.100982 &    -33.6 &            6.0 &      HIRES \\
2458781.095623 &    -11.0 &            5.9 &      HIRES \\
2458781.090310 &     11.5 &            6.2 &      HIRES \\
2458781.085102 &      0.9 &            5.8 &      HIRES \\
2458781.079696 &     15.7 &            6.0 &      HIRES \\
2458781.074082 &      9.3 &            6.0 &      HIRES \\
2458781.068550 &     33.3 &            5.7 &      HIRES \\
2458781.121967 &    -49.6 &            6.5 &      HIRES \\
2458780.916065 &    134.7 &            5.8 &      HIRES \\
2458780.947467 &    105.2 &            5.1 &      HIRES \\
2458780.881040 &    163.0 &            5.9 &      HIRES \\
2458780.858724 &    176.9 &            6.1 &      HIRES \\
2458780.869662 &    179.4 &            6.0 &      HIRES \\
2458780.886399 &    172.6 &            6.0 &      HIRES \\
2458780.853237 &    182.2 &            6.2 &      HIRES \\
2458780.864210 &    160.9 &            6.2 &      HIRES \\

2458787.981713 &   -371.2 &           10.0 &      HIRES \\
2458794.869141 &    -96.4 &            8.9 &      HIRES \\
2458795.906233 &    -34.9 &            8.3 &      HIRES \\
2458796.916527 &   -222.2 &            8.5 &      HIRES \\
2458797.953222 &    161.2 &            8.3 &      HIRES \\

2458780.873494 &    -82.0 &           16.0 &    PEPSI B \\
2458780.816464 &      4.0 &           14.0 &    PEPSI B \\
2458780.976136 &   -152.0 &           17.0 &    PEPSI B \\
2458781.010347 &   -135.0 &           18.0 &    PEPSI B \\
2458780.862084 &    -51.0 &           16.0 &    PEPSI B \\
2458781.033155 &   -164.0 &           19.0 &    PEPSI B \\
2458780.998944 &   -169.0 &           19.0 &    PEPSI B \\
2458780.839273 &     -1.0 &           14.0 &    PEPSI B \\
2458781.021751 &   -155.0 &           17.0 &    PEPSI B \\
2458780.827869 &     -3.0 &           15.0 &    PEPSI B \\
2458780.987539 &   -141.0 &           15.0 &    PEPSI B \\
2458780.964731 &   -136.0 &           17.0 &    PEPSI B \\
2458780.850680 &    -22.0 &           14.0 &    PEPSI B \\
2458780.793653 &      5.0 &           10.0 &    PEPSI B \\
2458780.919108 &   -174.0 &           21.0 &    PEPSI B \\
2458780.953327 &   -202.0 &           31.0 &    PEPSI B \\
2458780.884896 &    -82.0 &           17.0 &    PEPSI B \\
2458780.907705 &   -126.0 &           19.0 &    PEPSI B \\
2458780.782248 &     10.0 &           10.0 &    PEPSI B \\
2458780.941919 &    -88.0 &           23.0 &    PEPSI B \\
2458780.930514 &   -203.0 &           21.0 &    PEPSI B \\
2458780.805058 &     22.0 &           14.0 &    PEPSI B \\
2458780.770834 &      6.0 &           13.0 &    PEPSI B \\
2458780.896300 &    -91.0 &           19.0 &    PEPSI B \\
2458780.850663 &   -145.0 &           18.0 &    PEPSI R \\
2458781.033126 &   -479.0 &           22.0 &    PEPSI R \\
2458780.805047 &    -57.0 &           16.0 &    PEPSI R \\
2458780.782240 &      6.0 &           11.0 &    PEPSI R \\
2458780.827851 &   -128.0 &           18.0 &    PEPSI R \\
2458780.793643 &    -39.0 &           12.0 &    PEPSI R \\
2458780.816449 &    -49.0 &           17.0 &    PEPSI R \\
2458780.839256 &    -82.0 &           18.0 &    PEPSI R \\
2458780.770834 &     49.0 &           14.0 &    PEPSI R \\
2458780.919086 &   -299.0 &           25.0 &    PEPSI R \\
2458780.873468 &   -174.0 &           20.0 &    PEPSI R \\
2458780.930490 &   -335.0 &           26.0 &    PEPSI R \\
2458781.010320 &   -434.0 &           21.0 &    PEPSI R \\
2458780.896277 &   -226.0 &           23.0 &    PEPSI R \\
2458780.941892 &   -379.0 &           27.0 &    PEPSI R \\
2458780.998915 &   -375.0 &           23.0 &    PEPSI R \\
2458780.862066 &   -191.0 &           20.0 &    PEPSI R \\
2458781.021724 &   -410.0 &           21.0 &    PEPSI R \\
2458780.987510 &   -392.0 &           20.0 &    PEPSI R \\
2458780.907679 &   -285.0 &           24.0 &    PEPSI R \\
2458780.976106 &   -353.0 &           22.0 &    PEPSI R \\
2458780.964701 &   -410.0 &           22.0 &    PEPSI R \\
2458780.884873 &   -242.0 &           22.0 &    PEPSI R \\
2458780.953296 &   -442.0 &           35.0 &    PEPSI R \\
2458776.938191 &    -41.1 &           92.9 &       TRES \\
2458780.909176 &     -1.1 &           82.2 &       TRES \\
2458777.790792 &     51.6 &          110.6 &       TRES \\
2458774.881517 &    289.1 &          116.4 &       TRES \\
2458770.875874 &    -89.1 &          111.6 &       TRES \\
2458768.885490 &   -293.2 &           89.2 &       TRES \\
2458767.874876 &   -263.8 &          101.1 &       TRES \\
2458775.873139 &   -161.6 &          147.8 &       TRES \\
2458778.818078 &   -107.1 &           84.7 &       TRES \\
2458780.886651 &      1.1 &           73.8 &       TRES \\
2458780.747940 &    209.8 &           64.8 &       TRES \\
2458780.770343 &    157.2 &           95.1 &       TRES \\
2458780.933604 &     49.3 &          103.8 &       TRES \\
2458780.792717 &    219.4 &           81.0 &       TRES \\
2458780.955903 &     60.7 &           80.7 &       TRES \\
2458780.978699 &     18.0 &           71.2 &       TRES \\
2458780.837534 &    114.5 &           80.8 &       TRES \\
2458780.859931 &    105.5 &           86.8 &       TRES \\
2458781.000940 &    -68.4 &           73.8 &       TRES \\
2458781.023244 &    -67.7 &           92.8 &       TRES \\
2458779.930119 &   -233.9 &           95.9 &       TRES \\
\bottomrule
\end{tabular}

